A Graph Multi-separator Problem for Image Segmentation

We propose a novel abstraction of the image segmentation task in the form of a combinatorial optimization problem that we call the multi-separator problem. Feasible solutions indicate for every pixel whether it belongs to a segment or a segment separator, and indicate for pairs of pixels whether or not the pixels belong to the same segment. This is in contrast to the closely related lifted multicut problem where every pixel is associated to a segment and no pixel explicitly represents a separating structure. While the multi-separator problem is NP-hard, we identify two special cases for which it can be solved efficiently. Moreover, we define two local search algorithms for the general case and demonstrate their effectiveness in segmenting simulated volume images of foam cells and filaments.

==> sec_metrics.tex <==
To evaluate our proposed models for image segmentation we need measures to evaluate their performance.
For a given graph $G=(V,E)$ a separator $x: V \to \{0, 1\}$ let $X_1, \dots, X_k$ be the connected components of $G \setminus x^{-1}(1)$. 
Then we call the partition
\[
    P(x) = \bigl\{X_i \mid i \in \{1,\dots,k\}\bigr\} \cup \bigl\{\{v\} \mid v \in x^{-1}(1)\}
\]
of $V$ the  by $x$ \emph{induced partition}. 

Using the induced partitions of two multi separators $x$ and $y$ we can measure the distance of $x$ and $y$ by using classic distance measures for set partitions.
For example, we define the \emph{variation of information} for separators as
\[
    \vis(x, y) := \vi(P(x), P(y))
\]


\subsubsection*{Partial separators}

Training and evaluating a model for image segmentation requires labeled data. 
However, in practice, it might not be possible for experts to decide with certainty whether a given pixel belongs to the separator or not, for example, due to limited image quality. 
For that reason it can be advantageous to work with partially labeled data.
For that purpose we introduce the concept of partial separators.

\begin{definition}
    A \emph{partial separator} of a graph $G=(V,E)$ is a node labeling $x: V \to \{0, 1, *\}$ where for $v \in V$, $x_v = 0$ indicates that $v$ is not in the separator, $x_v = 1$ indicates that $v$ is in the separator and $x_v = *$ indicates that $x_v$ is ambiguous.

    A separator $x': V \to \{0,1\}$ is said to be \emph{consistent} with a partial separator $x$ if $x'_v = x_v$ for all $v \in V$ with $x_v \neq *$.
    We denote the set of all separators that are consistent with a partial separator $x$ by $C(x)$.
\end{definition}

For a distance measure $M$ on separators we can easily derive a distance measure $M_p$ on partial separators by defining
\begin{align}\label{eq:partial-dist-measure}
        M_p(x, y) := \min_{x' \in C(x), y' \in C(y)} M(x', y') \enspace ,
\end{align}
i.e. the minimal distance between any two separators $x'$ and $y'$ that are consistent with $x$ and $y$ respectively.
Notice that if there is a separator that is consistent with both $x$ and $y$ we have $M_p(x,y) = 0$.
As \eqref{eq:partial-dist-measure} is unsuitable to evaluate in practice we provide an explicit evaluation for the variation of information.

\begin{lemma}
    \todo{Can $\vis_p$ be computed efficiently? Probably not. Same for Rand?}
\end{lemma}

